Breaking Babel: A Self-Evolving Multi-Agent System for Long-Form Subtitle Translation

Long-form subtitle translation requires reasoning over discourse and cultural context spanning episodes or entire series, while maintaining consistent terminology and style. Existing single-LLM methods are largely sentence-level, and multi-agent systems often use static workflows that do not adapt to scene complexity or production context. We propose SMART, a Self-evolving Multi-Agent system for long-foRm subtitle Translation. During test-time training, SMART builds persistent series-level memory and translates a subset of sentences through a dynamic router and Mixture-of-Agents layer with tools for terminology verification, subtitle constraint validation, and contextual retrieval. A judge-refiner loop scores candidates and uses textual critiques to update agent prompts and routing policies without retraining the underlying LLMs. During test-time inference, the evolved configuration translates the remaining series. We also introduce Subtitle Arena, covering 14 genres, 2--198 episodes per series, production years 1959--2023, and 15 target locales, together with SubMQM, a subtitle-adapted MQM framework with seven dimensions and 19 error categories. SMART achieves the best overall MQM score in all 15 Subtitle Arena directions, reducing average penalty by 6.9% over the strongest competing agent system. On a public benchmark, MuSC, SMART obtains the best model result across all 4 language pairs. SMART also achieves the best result in human evaluation with an overall score of 4.50/5.

==> Secs/discussion.tex <==
% \textbf{Multimodal Expansion.}
% We extend SMART with video and audio tools powered by Qwen3-Omni~\citep{xu2025qwen3}. Across six representative directions, SMART + MM reduces the average AutoMQM penalty from 0.63 to 0.57 and outperforms the multimodal subtitle systems ViDove~\citep{lu2025vidove} and Hermes~\citep{cui2026hermes}. Full results are provided in Appendix~\ref{app:multimodal}.

% \textbf{Temporal Generalization.} On 200 TV series released in 2025--2026, including titles beyond the reported knowledge cutoff of Claude Sonnet 4.6, SMART outperforms TransAgent across all six evaluated directions. This suggests that its gains extend to temporally shifted content rather than being confined to Subtitle Arena. Details are in Appendix~\ref{sec:temporal-generalization}.

% \textbf{Qualitative Analysis.} Rendered examples further illustrate SMART's advantages on context-sensitive translation errors. Details are in  Appendix~\ref{app:rendered-frames}.


% \textbf{Multimodal Expansion.}
% Although SMART is designed primarily for text-based subtitle translation, its tool-augmented architecture naturally supports additional modalities. We therefore augment SMART with video and audio tools powered by Qwen3-Omni~\citep{xu2025qwen3}, allowing translators to selectively inspect aligned audiovisual sentences when textual context alone is insufficient. Across six representative translation directions, \textbf{SMART + MM consistently improves over text-only SMART}, reducing the average AutoMQM penalty from 0.63 to 0.57. The improvements are particularly pronounced for accuracy- and context-sensitive errors, suggesting that audiovisual evidence helps resolve ambiguities involving speaker intent, emotional delivery, and visually grounded references. SMART + MM also outperforms the multimodal subtitle systems ViDove~\citep{lu2025vidove} and Hermes~\citep{cui2026hermes} on all six directions. Full per-dimension results and implementation details are provided in Appendix~\ref{app:multimodal}.

% \textbf{Qualitative Analysis.}
% Penalties and rankings do not show what a viewer actually meets on screen, so we also inspect the outputs as rendered subtitles. We take six lines from the English$\rightarrow$Chinese passages of the human study and composite each system's subtitle onto the frame it plays over, at the position, size, and two-line budget a player would use, with the English source beneath it. Four failure modes of the baselines become visible in a single frame: a sarcastic idiom read as its opposite, a metaphor either deleted or transferred without being anchored in the target, an instrument of the source clause dropped, and a tradecraft term rendered with a general-purpose word. SMART is the only system that resolves the first two, and on the fourth it is the only one that reaches the idiomatic Chinese verb rather than a general-purpose synonym. The third is resolved by SMART, by Claude Opus 4.8, and by the agentic baseline TransAgent, but not by the single call to Claude Sonnet 4.6, which is SMART's own backbone: with the backbone held fixed, the difference is attributable to the scaffold rather than to the underlying model. The rendered comparisons and an indexed list of the lines are provided in Appendix~\ref{app:rendered-frames}.


